Cluster-Driven Expert Pruning for Mixture-of-Experts Large Language Models

Mixture-of-Experts (MoE) architectures have emerged as a promising paradigm for scaling large language models (LLMs) with sparse activation of task-specific experts. Despite their computational efficiency during inference, the massive overall parameter footprint of MoE models (e.g., GPT-4) introduces critical challenges for practical deployment. Current pruning approaches often fail to address two inherent characteristics of MoE systems: 1).intra-layer expert homogeneity where experts within the same MoE layer exhibit functional redundancy, and 2). inter-layer similarity patterns where deeper layers tend to contain progressively more homogeneous experts. To tackle these issues, we propose Cluster-driven Expert Pruning (C-Prune), a novel two-stage framework for adaptive task-specific compression of MoE LLMs. C-Prune operates through layer-wise expert clustering, which groups functionally similar experts within each MoE layer using parameter similarity metrics, followed by global cluster pruning, which eliminates redundant clusters across all layers through a unified importance scoring mechanism that accounts for cross-layer homogeneity. We validate C-Prune through extensive experiments on multiple MoE models and benchmarks. The results demonstrate that C-Prune effectively reduces model size while outperforming existing MoE pruning methods.

==> Ethic_Statement.tex <==
\section{}

==> experiment_1.tex <==
\section{Experiment}

\subsection{Experiment Setting}
\paragraph{Models and Infrastructure} We used DeepseekV2Lite (1 standard FFN + 26 MoE FFN layers) and Qwen1.5-MoE-A2.7B (24 MoE FFN layers) as our base models~\cite{deepseekv2, qwen_moe}. All experiments were conducted on a cluster of 32 NVIDIA A100 (80GB) GPUs.
\paragraph{Evaluation Protocol} Our evaluation covers three major benchmarks: MMLU~\cite{mmlu}, GSM8K~\cite{gsm8k}, and HumanEval~\cite{humaneval}, spanning computer science, mathematics, and business domains. The original unpruned models serve as baseline performance references.
\paragraph{Comparative Methods}
% To systematically evaluate the effectiveness of our pruning method, we established a multi-dimensional comparison framework: first, we used the unmodified original models \textbf{DeepSeek-V2-Lite} and \textbf{Qwen1.5-MoE-A2.7B} as performance benchmarks; second, 
We adopted the random pruning strategy proposed by \cite{random_pruning} as a basic reference; And, we introduced \textbf{SEER-MoE} method~\cite{seer_moe} and the similarity clustering-based \textbf{Group & Merge} method~\cite{group_merge}. 
% The former filters important experts through dynamic routing, while the latter merges redundant experts through feature space clustering, representing two typical paradigms of current MoE model compression.

% \subsection{Experiment Setting}
% \noindent \textbf{Studied Models}.
% For our pruning technique evaluation, we used DeepseekV2Lite~\cite{deepseekv2} with 1 standard FFN layer followed by 26 MoE FFN layers and Qwen1.5-MoE-A2.7B~\cite{qwen_moe} with 24 MoE FFN layers. All experiments were conducted on a distributed system of 32 NVIDIA A100 (80GB) GPUs.
% For our pruning technique evaluation, we used DeepseekV2Lite~\cite{deepseekv2} with 1 standard FFN layer followed by 26 MoE FFN layers (each having 2 shared experts and 64 routed experts, with 6 experts activated per token) and Qwen1.5-MoE-A2.7B~\cite{qwen_moe} with 24 MoE FFN layers (each containing 4 shared experts and 60 routed experts, with 4 experts activated per token).\\
% \noindent \textbf{Pruning methods}. We took two recent LLM expert pruning methods as our baseline. SEER-MoE~\cite{seer_moe} is a recent expert pruning technique that demonstrates its effectiveness when compared to \citet{lu2024not} on the Mixtral~\cite{jiang2024mixtral} series models. Its approach, which incorporates global pruning and leverages additional information from the routers in the MoE architecture, leads to significant improvements. On the other hand, \citet{moe_translate} focuses on identifying similarities between experts within each layer and directly merging them for future inference. However, both methods discard task-specific information and rely on a post-fine-tuning step to recover performance. \\
% In contrast, our method achieves state-of-the-art (SOTA) performance in task-specific experiments without requiring any fine-tuning stage. In fact, it even shows slight performance boosts in certain domains, as detailed in the Appendix. We continue to follow a data-centric{...} approach, but to capture expert similarities both layerwise and globally with traditional unsupervised learning techniques. Additionally, we investigate the effects of various pruning hyperparameters, which lead to improved performance across different domains. \\

% \subsection{Datasets}

% MMLU, HumanEval.GSM8K

% datasets fot inference:
% TIGER-Lab/MathInstruct
% @inproceedings{DBLP:conf/iclr/YueQZFH00C24,
%   author       = {Xiang Yue and
%                   Xingwei Qu and
%                   Ge Zhang and
%                   Yao Fu and
%                   Wenhao Huang and
%                   Huan Sun and
%                   Yu Su and
%                   Wenhu Chen},
%   title        = {MAmmoTH: Building Math Generalist Models through Hybrid Instruction
%                   Tuning},
%   booktitle    = {The Twelfth International Conference on Learning Representations,
%                   {ICLR} 2024, Vienna, Austria, May 7-11, 2024},
%   publisher    = {OpenReview.net},
%   year         = {2024},
%   url          = {https://openreview.net/forum?id=yLClGs770I},
%   timestamp    = {Mon, 29 Jul 2024 17:17:49 +0200},
%   biburl       = {https://dblp.org/rec/conf/iclr/YueQZFH00C24.bib},
%   bibsource    = {dblp computer science bibliography, https://dblp.org}
% }

% sahil2801/CodeAlpaca-20k
% @misc{codealpaca,
%   author = {Sahil Chaudhary},
%   title = {Code Alpaca: An Instruction-following LLaMA model for code generation},
%   year = {2023},
%   publisher = {GitHub},
%   journal = {GitHub repository},
%   howpublished = {\url{https://github.com/sahil280114/codealpaca}},
% }


% gbharti/finance-alpaca
% https://huggingface.co/datasets/gbharti/finance-alpaca


% each of which we took 1000 samples

% \paragraph{Baselines and Metrics}
% % 引用下测评的github（footnote）
% % Random, Seer, Group&Merge
% We established several baselines to assess the effectiveness of the pruning method. Initially, the original models, DeepSeek-V2-Lite~\cite{deepseekv2} and Qwen1.5-MoE-A2.7B~\cite{qwen_moe}, were used as the unpruned baseline, providing performance references without any structural modifications. In addition, we adopted a random pruning approach~\cite{random_pruning}, SEER-MoE~\cite{seer_moe} and the Group and Merge method~\cite{group_merge} based on expert similarity clustering as comparative baselines. These baselines were evaluated on multiple datasets including MMLU~\cite{mmlu}, GSM8K~\cite{gsm8k}, and HumanEval~\cite{humaneval}, covering tasks across the domains of computer science, mathematics, and business.

% \paragraph{Metrics}
% MMLU, Evalplus, GSM8K
% 引用下测评的github（footnote）


\subsection{Main Experiments}
% 简单对表格的结果进行分析：1. best method 2. task相关的体现出优势
\noindent \textbf{Efficient Pruning with Performance Balance}  
With a 20\% pruning rate, C-Prune reduces the parameter count of the DeepSeek model from 15.7B to 13.0B, while the MMLU composite score decreases by only 1.4\%, significantly outperforming random pruning (64\% performance drop). For the Qwen model, parameters are compressed from 14.3B to 11.8B, retaining 88\% of the MMLU score, as shown in Table~\ref{tab:repobench}.

\noindent \textbf{Robustness Across Domain-Specific Tasks}  
On computer science tasks, the pruned DeepSeek model achieves a score of 51.50, far surpassing baseline methods (e.g., Group\&Merge: 33.50). For mathematical reasoning, C-Prune outperforms the original model (DeepSeek: 33.56 vs. 32.21). In HumanEval, scores reach 18.90 (DeepSeek) and 32.90 (Qwen), highlighting advantages in technical domains.

\noindent \textbf{Limitations of Baseline Methods}  
Random pruning nearly fails on GSM8K tasks. While Group\&Merge approaches C-Prune in Qwen's business tasks, its overall performance gap remains significant (average score: 30.45 vs. 38.75), reflecting insufficient global optimization in existing methods.

\noindent \textbf{Gains from Task-Specific Fine-Tuning}  
Task-specific optimization mitigates performance loss effectively. For example, the pruned Qwen model achieves 39.40 on GSM8K (vs. 53.58 for the base model), a 56\% improvement over non-fine-tuned methods (Group\&Merge: 25.38), demonstrating deployment flexibility.

\noindent \textbf{Cross-Architecture Generalization}  
C-Prune maintains superior performance across both DeepSeek and Qwen. HumanEval scores remain close to base models (Qwen: 32.90 vs. 49.40), validating generalization capabilities across heterogeneous MoE architectures.



\begin{table*}[h]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{cccccccccccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Base Model} & \multirow{2}{*}{Parameters} & \multirow{2}{*}{Total Pruning Rate} & \multirow{2}{*}{\# of Routed Experts} & \multicolumn{4}{c}{MMLU} & \multirow{2}{*}{GSM8K} & \multirow{2}{*}{HumanEval} & \multirow{2}{*}{Average} \\ 
\cmidrule(lr){6-9}
 & & & & & Computer Science & Math & Business & Average & & & \\ 
\midrule
Base & DeepSeek-V2-Lite & 15.7B & 0 & 64 & 53.00 & 32.21 & 49.54 & 45.58 & 30.94 & 32.30 & 36.27 \\ 
Random & DeepSeek-V2-Lite & 13.0B & 0.2 & 52 & 19.00 & 12.32 & 17.53 & 16.28 & 0.057 & 0 & 5.446 \\ 
Seer Prune & DeepSeek-V2-Lite & 13.0B & 0.2 & 52 & 29.00 & 26.54 & 30.09 & 28.76 & 2.058 & 0 & 10.27 \\ 
Group\&Merge & DeepSeek-V2-Lite & 13.0B & 0.2 & 52 & 33.50 & 24.65 & 31.64 & 32.03 & 3.963 & 1.20 & 12.40 \\ 
\model{}(Ours) & DeepSeek-V2-Lite & 13.0B & 0.2 & 52 & \textbf{51.50} & \textbf{33.56} & \textbf{48.16} & \textbf{44.94} & \textbf{26.45} & \textbf{18.90} & \textbf{30.10} \\
\midrule
Base & Qwen1.5-MoE-A2.7B & 14.3B & 0 & 60 & 47.68 & 34.03 & 52.45 & 45.82 & 53.58 & 49.40 & 47.16 \\ 
Random & Qwen1.5-MoE-A2.7B & 11.8B & 0.2 & 48 & 14.50 & 13.81 & 11.04 & 13.12 & 10.44 & 12.90 & 12.15 \\ 
Seer Prune & Qwen1.5-MoE-A2.7B & 11.8B & 0.2 & 48 & 29.00 & 25.54 & 15.10 & 22.05 & 15.32 & 26.20 & 22.20 \\ 
Group\&Merge & Qwen1.5-MoE-A2.7B & 11.8B & 0.2 & 48 & 35.50 & 19.61 & \textbf{40.93} & 33.29 & 25.38 & 28.00 & 30.45 \\ 
\model{}(Ours) & Qwen1.5-MoE-A2.7B & 11.8B & 0.2 & 48 & \textbf{48.00} & \textbf{31.98} & 40.15 & \textbf{40.06} & \textbf{39.40} & \textbf{32.90} & \textbf{38.75} \\
\bottomrule
\end{tabular}%
}
\caption{Results of Model Evaluation on Benchmarks}
\label{tab:repobench}
\end{table*}


==> method.tex <==
\section{Methodology}

\noindent \textbf{Notations}.
We denote $F(\cdot;\Theta,W, K)$ as an MoE layer, where $\Theta=\{\theta_1, \theta_2,...,\theta_N\}$ indicates the parameter set for $N$ experts $\{f_{n}(\cdot;\theta_{n})\}_{n=1}^{N}$, $W\in\mathbb{R}^{N \times d}$ indicates the routing weights for each expert and $K$ indicates the number of experts selected for each token.  

For a new token $x\in \mathbb{R}^{d}$, we first compute the routing logits to score the match between $x$ and the $n$-th expert: 
\begin{equation}
    \begin{aligned}
        p_n(x) = \frac{e^{W_{n}x}}{\sum_{t=1}^{N}e^{W_{t}x}},
    \end{aligned}
\end{equation}
where $W_t\in\mathbb{R}^{d}$ is the routing policy of $t$-th expert.
Then, we take the experts $\{f_{n}(\cdot;\theta_{n})\}_{n=i_1}^{i_K}$ with top-$K$ logits $\{l_{n}\}_{n=i_1}^{i_K}$ as the selected target experts. Last, we compute the weighted average of the outputs from  selected experts as the final output of the MoE layer, 
\begin{equation}
    \begin{aligned}
        & y = \sum\limits_{n=i_1}^{i_K}p_n(x)\cdot f_{n}(x;\theta_{n}).\\
    \end{aligned}
\end{equation}

% /{\sum\limits_{t=i_1}^{i_k}l_{t}}
% \xd{we may directly use prob in eq 1. }

\subsection{Task Definition}

Previous works~\citep{lu2024not,he2024demystifying,li24merge} have identified that removing some experts from different MoE layers does not incur model collapse but improves efficiency in inference and fine-tuning on downstream tasks. The remaining question is which expert(s) should be pruned in the MoE layer.

Specifically, for the $l$-th MoE layer $F^{l}(\cdot; \Theta^l, W^l, K)$ in the given LLM $\mathcal{M}(\cdot;\mathcal{F})$, we want to prune  $r$ experts from the total of  $N$, $l=1,2,...,L$. This leads to the expert modules $\Theta$ being reduced to $\hat{\Theta}^l = \Theta^l \setminus \{\theta^l_{s^l_1}, \theta^l_{s^l_2}, \ldots, \theta^l_{s^l_r}\}$, and the routing matrix $W$ being reduced to $\hat{W}^l = W^l \setminus \{W^l_{s^l_1}, W^l_{s^l_2}, \ldots, W^l_{s^l_r}\}$, where $s^l = \{s^l_1, s^l_2, \ldots, s^l_r\}$ is the set of indices to delete. We aim to find the pruned $\hat{\mathcal{M}}$ by deleting the optimal indices set $s^l$ in different MoE layers $l$ towards the following optimization objective:

\begin{equation}
    \begin{aligned}
        \min\limits_{(x,y)\sim\mathcal{D}}\mathcal{L}(\hat{\mathcal{M}}(x;\hat{\mathcal{F}}),y),
    \end{aligned}\label{task:find_experts}
\end{equation}

where $\mathcal{L}$ is the loss function, $\hat{\mathcal{M}}(\cdot;\hat{\mathcal{F}})$ is the new LLM with pruned  MoE layer  $\hat{\mathcal{F}}$, and $\mathcal{D}$ is any dataset under the task-agnostic setting. 

This task is particularly challenging, as this is an NP-hard search problem with \((C^{r}_{N})^L\) possible solutions. In this work, we propose to estimate the expert similarity in the feature space for greedy structured pruning within each MoE layer to address this problem.

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/framework.pdf}
    \caption{Evaluation of the expert similarity for different MoE layers in Mixtral-8x7B under two kernel-based CKA criteria (Linear and RBF). A darker color indicates a greater similarity between experts. }
    \label{fig:motivation_mixtral_experts}
\end{figure*}




\subsection{Expert Similarity in MoE Layer}
\label{sec:motivation}

\noindent \textbf{Motivation}: Intuitively, the more independent the experts are within the same MoE layer, the more diverse the representations learned by each expert. This diversity makes it harder to replace or drop any of the experts. Conversely, the redundancy of shared knowledge learned by different experts provides opportunities for model pruning.

To evaluate the similarity between experts, we compute the cosine similarity of the embeddings obtained from each expert. Specifically, given a batch of inputs $\{x_1, x_2, ..., x_s\}$, the embedding of expert $f_i$ for input $x_m$ is denoted as $\mathcal{M}(f_i(x_m))$, where $m = 1, 2, \ldots, s$. The similarity $\rho_{ij}$ between two experts $f_i$ and $f_j$ is calculated by the cosine similarity of their embeddings:

\begin{equation}
    \rho_{ij} = \frac{\mathcal{M}(f_i(x_m)) \cdot \mathcal{M}(f_j(x_m))}{\|\mathcal{M}(f_i(x_m))\| \|\mathcal{M}(f_j(x_m))\|},
\end{equation}
where $\mathcal{M}(f_i(x_m))$ is the embedding of expert $f_i$ for input $x_m$.

In this work, we use the embedding of each expert after processing a batch of inputs as their feature representation and compute the cosine similarity across all pairs of experts.

For further analysis, we compute the expert similarity for Mixtral-8Bx7B using a randomly selected set of $32$ samples from the pre-trained C4 dataset~\citep{raffel2020exploring}. The similarity computation uses the cosine similarity of the expert embeddings for each of the selected samples. We apply this method with both the linear kernel and RBF kernel to assess the similarity between expert embeddings. 

As illustrated in Fig.~\ref{fig:motivation_mixtral_experts}, the darker the cell, the more similar the two related experts. The similarity patterns using both the linear and RBF kernels show similar changes in expert similarity across different layers. We observe varying ratios of similar expert pairs in different MoE layers, suggesting the plausibility of pruning MoE layers with many experts down to fewer experts.


\subsection{Layerwise Pruning Process}

In Layerwise Pruning, we first compute the embeddings of each expert. Then, hierarchical clustering is applied to these embeddings to group similar experts together. The algorithm for this step is as follows:

\begin{itemize}
    \item Compute the embedding $\mathcal{M}(f_n)$ for each expert $f_n$.
    \item Apply hierarchical clustering to these embeddings to form $r$ clusters of experts. 
    \item For each cluster, we prune a certain proportion of experts based on their similarity to others in the same cluster.
\end{itemize}

Hierarchical clustering can be mathematically described as follows. Given a set of expert embeddings $\{\mathcal{M}(f_1), \mathcal{M}(f_2), \ldots, \mathcal{M}(f_N)\}$, we build a similarity matrix $D \in \mathbb{R}^{N \times N}$, where $D_{ij}$ is the pairwise similarity between expert $f_i$ and $f_j$. We apply agglomerative hierarchical clustering, where the goal is to minimize the following objective function:

\begin{equation}
    \min \sum_{i=1}^{r} \left( \sum_{j,k \in \mathcal{V}_i} D_{jk} - \sum_{t \neq i}^{r} \sum_{j \in \mathcal{V}_i, k \in \mathcal{V}_t} D_{jk} \right),
\end{equation}
where $\mathcal{V}_i$ is the set of expert indices in the $i$-th cluster. This optimization minimizes the intra-cluster similarity and maximizes the inter-cluster difference.

\subsection{Global Pruning Process}

After Layerwise Pruning, we proceed with Global Pruning. In this step, we compute the embeddings of the remaining experts and apply hierarchical clustering across all MoE layers. This step follows the same approach as Layerwise Pruning, but with the entire set of remaining experts from all layers:

\begin{itemize}
    \item Compute the embeddings for the remaining experts after Layerwise Pruning.
    \item Apply hierarchical clustering across the remaining experts to form $r$ clusters.
    \item Prune experts from each cluster based on their similarity to others.
\end{itemize}

The hierarchical clustering step for global pruning involves the same objective as in Layerwise Pruning but now across all remaining experts, which can be formulated as:

\begin{equation}
    \min \sum_{i=1}^{r} \left( \sum_{j,k \in \mathcal{V}_i} D_{jk} - \sum_{t \neq i}^{r} \sum_{j \in \mathcal{V}_i, k \in \mathcal{V}_t} D_{jk} \right),
\end{equation}
where the clustering is done across all remaining experts from all MoE layers.

\subsection{Pruning Algorithm}

The overall pruning algorithm proceeds as follows:

\begin{itemize}
    \item First, compute the embeddings of all experts.
    \item Apply hierarchical clustering to group experts based on their similarity.
    \item For each cluster, prune experts according to their similarity.
    \item For the Layerwise Pruning, prune experts within each MoE layer.
    \item For the Global Pruning, prune experts across all layers.
\end{itemize}

After clustering, the experts in each cluster are merged into a single expert by averaging their weights and routing policies:

\begin{equation}
    \hat{\theta}_{n} \leftarrow \sum_{i=1}^{|\mathcal{V}_n|} \alpha_{i} \theta_{\mathcal{V}_n(i)}, \quad \hat{W}_n \leftarrow \sum_{i=1}^{|\mathcal{V}_n|} \alpha_{i} W_{\mathcal{V}_n(i)},
\end{equation}
where $\alpha_i$ is a weighting factor for each expert in the cluster.

Finally, the MoE layer is updated by replacing the experts in each cluster with a single merged expert, and the routing weights are adjusted accordingly.

